Sign Stitching: A Novel Approach to Sign Language Production

Sign Language Production (SLP) is a challenging task, given the limited resources available and the inherent diversity within sign data. As a result, previous works have suffered from the problem of regression to the mean, leading to under-articulated and incomprehensible signing. In this paper, we propose using dictionary examples to create expressive sign language sequences. However, simply concatenating the signs would create robotic and unnatural sequences. Therefore, we present a 7-step approach to effectively stitch the signs together. First, by normalising each sign into a canonical pose, cropping and stitching we create a continuous sequence. Then by applying filtering in the frequency domain and resampling each sign we create cohesive natural sequences, that mimic the prosody found in the original data. We leverage the SignGAN model to map the output to a photo-realistic signer and present a complete Text-to-Sign (T2S) SLP pipeline. Our evaluation demonstrates the effectiveness of this approach, showcasing state-of-the-art performance across all datasets.

==> Sections/4_setup.tex <==
% \subsubsection{Implementation Details}
\textbf{Implementation Details:} In our experiments, we conducted a grid search for optimal hyper-parameters and identified the following settings as the most effective. Our encoder-decoder translation model is constructed with an embedding size of 512 and a feed-forward size of 1024. We find that the optimal number of layers and heads is dataset-dependent, with smaller datasets requiring fewer layers compared to \ac{mdgs} where we use 3 layers and 4 heads. The models utilise dropout with a probability of 0.1 \cite{srivastava2014dropout}, ReLU activations between layers \cite{agarap2018deep}, and pre-layer normalisation for regularisation and training stability. Training employs a 'reduce on plateau' scheduler with a patience of 5 and a decrease factor of 0.8. The layers are initialised using a Xavier initializer \cite{glorot2010understanding} with zero bias, and during training, Adam optimization is employed \cite{kingma2014adam}.  The initial learning rate is set to \(10^{-4}\), and we train the model until convergence. During decoding, we utilise a greedy search algorithm. The loss scaling factors, \(\lambda_{y}\), \(\lambda_{d}\), \(\lambda_{f}\) and \(\lambda_{C}\) are set to 1.0, 0.1, 0.3 and 0.2, respectively.  
When stitching we enforce a minimum sign length, \(U_{min}\) of 4 frames. The cropping threshold, \(\alpha_{crop}\) is dataset-dependent, we find values between the range of 0.1 to 0.35 most effective. All sequences are subsampled to 12 \ac{fps} for computational efficiency. 

For each dataset, we create a dictionary of 500 facial expressions. We scale the counter loss by 0.01 and we set an embedding dimension of 512. The encoder and decoder are initialized with the same settings as our translation model. 

The angular pose representation comprises 104 angles, while the Euclidean representation consists of 61 keypoints (21 for each hand and 19 for the body and face). The face mesh we add includes 128 keypoints, which are a subset of Mediapipe's 478-face mesh \cite{lugaresi2019mediapipe}.

For comparison, we train a progressive transformer on each dataset until convergence using the parameters from \cite{saunders2020progressive}.

\textbf{Datasets:} The approach is tested on three datasets, the Public Corpus of
German Sign Language, 3rd release, the \ac{mdgs} dataset \cite{dgscorpus_3}, \ac{ph14t} \cite{camgoz2018neural} and the \ac{bslcpt} \cite{schembri2008british}. \ac{bslcpt} contains 211 participants from 8 regions in the UK, performing 4792 individual signs from a range of age groups. The participants perform narrative, interviews and participate in free conversation. Similarly, \ac{mdgs} contains 330 participants engaging in free-form signing. Whereas, the \ac{ph14t} dataset is extracted from German TV weather broadcasters and contains over 8,000 parallel sequences. 

\textbf{Dictionary:} In the following experiment, we test two different dictionaries: 1) collected from isolated examples, and 2) a dictionary created from continuous data. Next, we provide further details about each:


Isolated - Here, the signs are sourced from individuals who perform each sign in isolation, typically starting from and returning to a resting position. When experimenting on the \ac{bslcpt} we use the Signbank dataset \cite{cormier2012corpus}, it contains over 3,000 signs and includes all the lexical variants found in the \ac{bslcpt} dataset. However no such dictionary exists for the \ac{ph14t} and \ac{mdgs} dataset, therefore we collect a dictionary from a range of sources such as \cite{dgscorpus_3}. We find the \ac{mdgs} dataset has a target vocabulary of 10,801. However, without the gloss variant, we find the core gloss vocabulary reduces to 4,434. We collect a total of 7,206 signs to experiment with. We use the method described in \cref{sec:methodology} (Stitching), step 1 to overcome issues with an incomplete vocabulary. To create word embeddings we apply Facebook's implementation of Fasttext \cite{mikolov2013distributed}. When experimenting on the \ac{bslcpt} we use the English implementation whereas on \ac{ph14t} and \ac{mdgs} we use the German implementation.

Continuous - Here we create a dictionary using the gloss timing annotations. The signs are taken from the test and dev data only, so that the back translation model has not seen the signs during training. As the examples come from the continuous sign, we omit the cropping step of the stitching pipeline. These dictionaries have an abundance of signs to choose from when stitching.
We filter the dictionary and remove short signs as these are most likely co-articulated and therefore not suitable or out of context. We opt to randomly select the first sign in the sequence, and subsequent signs are chosen to ensure the most natural transition. Therefore, we select the sign from the dictionary in which the location of the wrist is closest to the last frame of the previous sign.

\textbf{Evaluation Metrics:} To evaluate our approach we employ a \ac{cslr} model (Sign Language Transformers \cite{camgoz2020sign}) to conduct back-translation, the same as \cite{huang2021towards, saunders2020adversarial, saunders2021mixed, xie2022vector}. A model is trained for each dataset and the parameters are frozen so that results are consistent. BLEU \cite{papineni2002bleu}, Rouge \cite{lin2004rouge}, and chrF \cite{popovic-2015-chrf} scores are computed between the predicted text and the ground truth. To evaluate the pose we employ \ac{dtwmje}, the metric compresses and stretches time to find the best alignment between the ground truth, \(p\), and the predicted pose, \(\hat{p}\). 


==> Tables/table_template.tex <==
\begin{table*}
\centering
\caption{\label{tab:mdgs_abalation}The results of translating from Text-to-Pose on the BSL Corpus \textbf{T} dataset.}
\resizebox{\linewidth}{!}{%

\begin{tabular}{r|cccccc|cccccc} 
\toprule
\multicolumn{1}{l}{BSLCP\textbf{T}}      & \multicolumn{7}{c}{TEST SET}       & \multicolumn{7}{c}{DEV SET}  \\
\multicolumn{1}{c|}{Approach:} & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & chrF & ROUGE & WER & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & chrF & ROUGE & WER  \\ 
\midrule
GT              & 0.000    &        &        &        &        &      &       &     & 0.000   &        &        &        &        &      &       &     \\
PT              &          &        &        &        &        &      &       &     &         &        &        &        &        &      &       &     \\
PT + GN         &          &        &        &        &        &      &       &     &         &        &        &        &        &      &       &     \\
Stitcher (ours) &          &        &        &        &        &      &       &     &         &        &        &        &        &      &       &     
\bottomrule
\end{tabular}
}
\end{table*}
